ARviz -- An Augmented Reality-enabled Visualization Platform for ROS Applications

Current robot interfaces such as teach pendants and 2D screen displays used for task visualization and interaction often seem unintuitive and limited in terms of information flow. This compromises task efficiency as interacting with the interface can distract the user from the task at hand. Augmented Reality (AR) technology offers the capability to create visually rich displays and intuitive interaction elements in situ. In recent years, AR has shown promising potential to enable effective human-robot interaction. We introduce ARviz - a versatile, extendable AR visualization platform built for robot applications developed with the widely used Robot Operating System (ROS) framework. ARviz aims to provide both a universal visualization platform with the capability of displaying any ROS message data type in AR, as well as a multimodal user interface for interacting with robots over ROS. ARviz is built as a platform incorporating a collection of plugins that provide visualization and/or interaction components. Users can also extend the platform by implementing new plugins to suit their needs. We present three use cases as well as two potential use cases to showcase the capabilities and benefits of the ARviz platform for human-robot interaction applications. The open access source code for our ARviz platform is available at: https://github.com/hri-group/arviz.

==> Text/tfListener.tex <==
For example, PointCloud data collected from a camera needs to be positioned with respect to the camera frame. The location of the camera frame must be known in order to correctly visualize the data received from the camera. In ROS, this information is kept track by the tf package, in which ROS programmers can access using tf Listener Application Programming Interface (API) provided with the tf package. However, as \textbf{ARviz} was built on Unity Game Engine which does not support ROS natively, the platform does not have access to this API to obtain the transformation frames data. To solve this issue, we implement our own version of tf Listener in Unity. Coordinate frames and transformations between them are published to \textit{/tf} and \textit{/tf\_static} respectively, in the form of TF Message. TF Message is collection of coordinate frame transformations which specifies the origin of a frame a.k.a its parent frame, as well as the relative position and orientation of that frame from its parent a.k.a transformation between two frames. \textbf{Unity tf Listener} uses these messages obtained from these two subscribers to build a hierarchical structure with every elements in the hierarchy being positioned at where the TF messages specified. With this data structure, other components on the platform will have access to any reference points in the hierarchy to place their visual elements appropriately. This hierarchical structure is updated every 20ms, allowing a near real-time update on the positions of these frames for more accurate placement of the visual elements. 
